A Deep Reinforcement Learning Approach towards Pendulum Swing-up Problem based on TF-Agents

Adapting the idea of training CartPole with Deep Q-learning agent, we are able to find a promising result that prevent the pole from falling down. The capacity of reinforcement learning (RL) to learn from the interaction between the environment and agent provides an optimal control strategy. In this paper, we aim to solve the classic pendulum swing-up problem that making the learned pendulum to be in upright position and balanced. Deep Deterministic Policy Gradient algorithm is introduced to operate over continuous action domain in this problem. Salient results of optimal pendulum are proved with increasing average return, decreasing loss, and live video in the code part.

==> problem.tex <==
\newtheorem{myDef}{Definition}

\section{Problem Statement}
\label{sec:problem}

In this section, we formally present the problem of multimodal COVID-19 news credibility assessment. We first define a few key terms that will be used in the problem statement. 

\begin{myDef}
\emph{\textbf{COVID-19 News Post ($\mathcal{P}_i$):} A COVID-19 news post $\mathcal{P}_i$ refers to an online multimodal news post that is related to COVID-19. In particular, each COVID-19 news post includes two components: \textit{news text} and \textit{news image}.
\begin{itemize}
    \item \textbf{News Text ($\mathcal{T}_i$):} the text of the news post that depicts the news event or topic.
    \item \textbf{News Image ($\mathcal{I}_i$):} the image in the news post that is relevant to the news event or topic discussed in the post.
\end{itemize}
}
\end{myDef}


\begin{myDef}
\emph{\textbf{News Credibility ($y_i$):} \lanyu{We consider two categories of news credibility (i.e., true or false) in our study.
A COVID-19 news post is \textit{false} (i.e., $y_i=0$) if the news text and news image jointly deliver misleading content (e.g., false information, conspiracy claim, irrelevant content). Otherwise, the news post is considered to be \textit{true} (i.e., $y_i=1$).}
}
\end{myDef}

Our goal is to assess the credibility of the multimodal COVID-19 news posts by classifying the posts into two categories \lanyu{(i.e., true or false)}. In particular, we assume a set of $N$ COVID-19 multimodal news posts $\mathcal{P} = \{\mathcal{P}_1, \mathcal{P}_2, \cdots, \mathcal{P}_N\}$. For each $\mathcal{P}_i \in \mathcal{P}$, our objective is: 

\begin{equation}
    \argmax_{\hat{y_i}} \Pr (\hat{y_i}=y_i | \mathcal{P}_i), \forall~ 1\leq i \leq N
\end{equation}
\noindent
where $y_i$ and $\hat{y_i}$ are the ground truth and estimated label of the COVID-19 news post $\mathcal{P}_i$, respectively. 

==> relatedwork.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Online Information Credibility Assessment}
The credibility of online information has raised many concerns in recent years, especially for the user-generated content on social media~\cite{nelson2021improve}.
Many efforts have been made to assess the credibility of information online. 
For example, Popat \textit{et al.} proposed the CredEye system that assesses the credibility of social media claims by exploiting the language style and stance characteristics of the textual content~\cite{popat2018credeye}.
Mukherjee~\textit{et al.} developed a probabilistic graphical model to examine the credibility of user-generated statements on online health communities~\cite{mukherjee2014people}.
Horne \textit{et al.} designed an online news credibility assessment tool for analyzing the credibility of online news articles using a set of hand-crafted features (e.g., reliability of the news source, content subjectivity)~\cite{horne2018assessing}.
However, existing approaches for news credibility assessment often rely on the news content (e.g., language style) or auxiliary information (e.g., users' sentiments) to identify false or misleading information.
% external or contextual information (e.g., users' sentiment. 
Such kind of information is not necessarily reliable to assess the news credibility, especially for the news posts that are intentionally crafted to mislead the audience who often lack professional knowledge to make reliable decisions~\cite{vraga2017using}. 
% of intentionally crafted news, especially when our knowledge of a breaking event (e.g., the outbreaking of COVID-19) is limited~\cite{vraga2017using}. 
% In this paper, we propose a novel generative approach to assess the credibility of multimodal COVID-19 news by inferring consistency between the generated and original textual/visual content of the  multimodal COVID-19 news.



\subsection{Generative Learning}
Our work is also closely related to generative learning, which has been applied in many applications including image synthesis, recommender systems
% ~\cite{deldjoo2021survey}, 
and speech generation
% ~\cite{zhang2020adversarial}
~\cite{pan2019recent}. 
More recently, generative learning has been applied to study online misinformation. 
For example, Zellers \textit{et al.} developed a generative adversarial network (GAN) based fake news discriminator to identify machine generated fake news~\cite{zellers2019defending}.
Similarly, Yanagi \textit{et al.} proposed a generative fake news detector to identify fake news using comments automatically generated from the news content~\cite{yanagi2020fake}.
Ma \textit{et al.} designed a GAN-style rumor detection method that learns the discriminative patterns between rumor and non-rumor posts on social media~\cite{ma2019detect}. However, these solutions ignore the interdependence between textual and visual information in multimodal news which is fundamental in assessing the credibility of COVID-19 news with exaggerated or irrelevant content. 
% In this paper, we present a duo-generative framework that leverages the image and text respectively generated from the news text and news image to capture the interdependence between different modalities for assessing the credibility of multimodal COVID-19 news.   





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% multimodal 
